A Survey on Reinforcement Learning Methods in Character Animation

Reinforcement Learning is an area of Machine Learning focused on how agents can be trained to make sequential decisions, and achieve a particular goal within an arbitrary environment. While learning, they repeatedly take actions based on their observation of the environment, and receive appropriate rewards which define the objective. This experience is then used to progressively improve the policy controlling the agent's behavior, typically represented by a neural network. This trained module can then be reused for similar problems, which makes this approach promising for the animation of autonomous, yet reactive characters in simulators, video games or virtual reality environments. This paper surveys the modern Deep Reinforcement Learning methods and discusses their possible applications in Character Animation, from skeletal control of a single, physically-based character to navigation controllers for individual agents and virtual crowds. It also describes the practical side of training DRL systems, comparing the different frameworks available to build such agents.

==> tables/algorithms-old.tex <==
\begin{table*}[ht]\centering
\caption{A summary of the DRL algorithms, simulation engines, and neural network frameworks in the described papers, where applicable and stated in the paper or the provided source code. $^{1}$ Temporal Difference learning, $^{2}$ Maximum A Posteriori Policy Optimization, $^{3}$ Open Dynamics Engine, $^{4}$ Value Iteration.}\label{tab:algorithms}
\begin{tabular}{ccccc}
Citation                           & Year & Algorithm    & Physics Simulation Engine & NN Framework \\ \hline
\cite{liu2017learning}             & 2017 & DQN          & ODE$^{3}$                       & Theano       \\
\cite{liu2018learning}             & 2018 & DDPG         & ODE$^{3}$                       & Theano       \\
\cite{peng_deeploco_2017}          & 2017 & TD$^{1}$           & --                         & --            \\
\cite{peng_deepmimic_2018}         & 2018 & PPO          & Bullet                    & TensorFlow   \\
\cite{peng2020learning}            & 2020 & PPO          & Bullet                    & TensorFlow   \\
\cite{peng2018sfv}                 & 2018 & PPO          & Bullet                    & TensorFlow   \\
\cite{peng2017learning}            & 2017 & TD           & --                         & --            \\
\cite{peng_amp_2021}               & 2021 & PPO + GAIL   & Bullet                    & TensorFlow   \\
\cite{chentanez2018physics}        & 2018 & PPO          & MuJoCo                    & TensorFlow   \\
\cite{park2019learning}            & 2019 & PPO          & DART                      & TensorFlow   \\
\cite{bergamin2019drecon}          & 2019 & PPO          & Bullet                    & TensorFlow   \\
\cite{wang2020unicon}              & 2020 & PPO          & Flex                      & -            \\
\cite{won2020scalable}             & 2020 & PPO          & Bullet                    & TensorFlow   \\
\cite{lee2019scalable}             & 2019 & PPO          & DART                      & PyTorch      \\
\cite{won2019learning}             & 2019 & PPO          & DART                      & TensorFlow   \\
\cite{lee2021learning}             & 2021 & PPO          & DART                      & TensorFlow   \\
\cite{ma2021learning}              & 2021 & PPO          & Bullet                    & PyTorch      \\
\cite{yuan2020residual}            & 2020 & PPO          & MuJoCo                    & PyTorch      \\
\cite{merel2020catch}              & 2020 & V-MPO$^{2}$        & MuJoCo                    & NumPy        \\
\cite{luo_carl_2020}               & 2020 & PPO          & Bullet                    & TensorFlow   \\
\cite{Ling2020}                    & 2020 & PPO          & Bullet                    & PyTorch      \\
\cite{isogawa_optical_2020}        & 2020 & PPO          & MuJoCo                    & TensorFlow   \\
\cite{yuan_simpoe_2021}            & 2021 & PPO          & MuJoCo                    & PyTorch      \\
\cite{peng_dynamic_2015}           & 2015 & VI$^{4}$           & Box2D                     & -            \\
\cite{peng_terrain-adaptive_2016}  & 2016 & CACLA        & Bullet                    & Caffe        \\
\cite{yu_learning_2018}            & 2018 & PPO          & DART                      & TensorFlow   \\
\cite{abdolhosseini_learning_2019} & 2019 & PPO          & Bullet, MuJoCo            & PyTorch      \\
\cite{xie_allsteps_2020}           & 2020 & PPO          & Bullet                    & PyTorch      \\
\cite{kumar_learning_2017}         & 2017 & CACLA        & DART                      & Caffe        \\
\cite{clegg_learning_2018}         & 2018 & TRPO         & DART                      & PyTorch      \\
\cite{yin_discovering_2021}        & 2021 & PPO          & Bullet                    & PyTorch      \\
\cite{long_towards_2018}           & 2018 & IPPO         & Stage                     & TensorFlow   \\
\cite{lee_crowd_2018}              & 2018 & IDDPG        & --                         & TensorFlow   \\
\cite{xu_local_2020}               & 2020 & IPPO + ORCA  & --                         & PyTorch      \\
\cite{sun_crowd_2019}              & 2019 & IPPO + RVO   & Unity3D                   & --            \\
\cite{haworth_deep_2020}           & 2020 & IPPO, MADDPG & Bullet                    & Caffe        \\
\cite{huttenrauch_deep_2019}       & 2019 & ITRPO        & --                         & TensorFlow   \\
\cite{alonso_deep_2020}            & 2020 & SAC          & Unity3D                   & --            \\
\cite{zou_understanding_2018}      & 2018 & TRPO + GAIL  & --                         & TensorFlow   \\
\cite{xu_human-inspired_2021}      & 2021 & IPPO         & --                         & PyTorch     
\end{tabular}
\end{table*}

==> text/bios.tex <==
Ariel Kwiatkowski is a doctoral student and an Early Stage Researcher in the CLIPE ITN, a project funded under the Marie Skłodowska-Curie Actions program. He gained his Bachelor's degree in Physics (Individual Track) at University of Warsaw, with his thesis being about applications of Machine Learning to the field of atmospheric physics. Then he obtained a double Master's degree from KTH Royal Institute of Technology and Aalto University, under the EIT Digital Master School, with a major in Autonomous Systems. His Master's Thesis explored agents modelling one another in a multiagent reinforcement learning scenario. Now he works towards his PhD at École Polytechnique, applying multiagent reinforcement learning methods to crowd simulation, seen as part of computer graphics. He actively contributes to open-source software commonly used in reinforcement learning such as OpenAI Gym, PettingZoo or SuperSuit. His other research interests include emergent phenomena in intelligent systems, AI alignment and physics-informed reinforcement learning.

Eduardo Alvarado is a second-year doctoral student in the Geometric & Visual Computing (GeoViC) group at École Polytechnique, and an Early Stage Researcher as part of the Marie Skłodowska-Curie Innovative Training Network CLIPE, funded by the European Union for the Horizon 2020 framework. He is supervised by Prof. Damien Rohmer and Prof. Marie-Paule Cani. Prior to his PhD, Eduardo gained his Bachelor's degree in Electronics Engineering at Universidad Carlos III in Madrid, and wrote his thesis on Geolocalization-based Augmented Reality. He then obtained his Master's degree in Embedded Systems Engineering at Albert-Ludwigs-Universität Freiburg, with a major in Deep Learning, Reinforcement Learning and Computer Vision for Robotics. During this time, he worked extensively in the field of Autonomous Driving, both academically and in industry for companies such as ZF Friedrichshafen or Robert Bosch GmbH, where he wrote his thesis on Deep Multi-modal Learning for Sensor-Fusion under the supervision of Prof. Joschka Boedecker and Prof. Abnihav Valada. Now, he works towards his PhD in real-time animation synthesis. His research is centered on multi-scale animation methods for humans and quadrupeds in dynamic and outdoor environments, interactive use of AI for authoring virtual content and understanding/improving user-experience on real-time applications.

Vicky Kalogeiton is an Assistant Professor in the Computer Science Laboratory at École Polytechnique, where she is part of the GeoViC team. Before, she was a research fellow at VGG, the University of Oxford. She completed her PhD in 2017 at the CALVIN group, University of Edinburgh and the THOTH team (previous name LEAR), INRIA Grenoble. Her research interests are computer vision with deep learning and specifically human-centric video understanding.

C. Karen Liu is an associate professor in the Computer Science Department at Stanford University. Prior to joining Stanford, Liu was a faculty member at the School of Interactive Computing at Georgia Tech. She received her Ph.D. degree in Computer Science from the University of Washington. Liu's research interests are in computer graphics and robotics, including physics-based animation, character animation, optimal control, reinforcement learning, and computational biomechanics. She developed computational approaches to modeling realistic and natural human movements, learning complex control policies for humanoids and assistive robots, and advancing fundamental numerical simulation and optimal control algorithms. The algorithms and software developed in her lab have fostered interdisciplinary collaboration with researchers in robotics, computer graphics, mechanical engineering, biomechanics, neuroscience, and biology. Liu received a National Science Foundation CAREER Award, an Alfred P. Sloan Fellowship, and was named Young Innovators Under 35 by Technology Review. Liu also received the ACM SIGGRAPH Significant New Researcher Award for her contribution in the field of computer graphics. In 2021, Liu was inducted to ACM SIGGRAPH Academy.

Julien Pettré is a computer scientist. He is senior researcher at Inria, the French National Institute for Research in Computer Science and Control, in the Rainbow team. He received PhD from the University of Toulouse III in 2003, and Habilitation from the University of Rennes I in 2015. From 2004 to 2006, he was postdoctoral fellow at EPFL in Switzerland. He joined Inria in 2006.
Julien Pettré is currently coordinator of the European H2020 Crowdbot project (2018-21) dedicated to the design of robot navigation techniques for crowded environments. He is also the coordinator of the European H2020 Fet Open CrowdDNA project (2020-2024), dedicated to future emergent technologies for crowd management in public spaces. He previously coordinated the national ANR JCJC Percolation project (2013-17) dedicated to the design of new microscopic crowd simulation algorithms, as well as the national ANR CONTINT Chrome project, dedicated to efficient and designer-friendly techniques for crowd animation.
His research interests are crowd simulation, computer animation, virtual reality, robot navigation and motion planning.

Michiel van de Panne's research interests are in deep reinforcement learning, physics-based models of human and animal movement, motion planning and control, robotics, and applications of machine learning to computer graphics. He is Professor in the Department of Computer Science at the University of British Columbia. He is deputy director of CAIDA, UBC's main AI organization. In 2002 he co-founded the ACM/Eurographics Symposium on Computer Animation, a leading forum for computer animation research. He has served as Associate Editor of ACM Transactions on Graphics and regularly serves on numerous program committees. His former students and postdocs have (co)founded four companies, hold leadership positions in others, and are faculty at numerous universities worldwide.

Marie-Paule Cani is a Professor of Computer Science at Ecole Polytechnique. Her research interests cover both Shape Modelling and Computer Animation. She contributed over the years to a number of high level models for shapes and motion such as implicit surfaces, multi-resolution physically-based animation methods and hybrid representations for real-time natural scenes. Following a long lasting interest for virtual sculpture, she has been recently searching for more expressive ways to create 3D contents such as combining sketch-based interfaces with procedural models based on a priori knowledge or learning. She received the Eurographics outstanding technical contributions award in 2011, a Silver medal from CNRS in 2012, and was elected at the Academia Europaea in 2013. She was awarded the ERC advanced grant EXPRESSIVE (2012-2017) and joined the ACM Siggraph Academy in 2019. She was elected at the French Academy of Sciences in 2020.
Marie-Paule Cani was the Technical Paper Chair of ACM SIGGRAPH 2017, and program co-chair of Motion, Interaction and Games (MIG) in 2019. Before that, she served in the program committees of all major conferences in computer graphics and was program chair a number of times. She served in the steering committees of SCA, SBIM and SMI, and in the editorial board of ACM Transactions of Graphics (TOG), Computer Graphics Forum, IEEE TVCG and Graphical Models. She is now associate editor of Computers and Graphics. She was Director at Large in the EC of ACM SIGGRAPH from 2007 to 2011, and member of the ACM Publication Board from 2011 to 2014. In France, she served in the executive board of the GDR IG-RV (Informatique Géométrique et Graphique, Réalité Virtuelle et Visualisation) of CNRS and in the CA of the French chapter of Eurographics for many years. After being vice president from 2013, she was President of the Eurographics association in 2017 and 2018.
